Search for charged long-lived particles at the Future Circular Collider (FCC-ee)

Long-lived particles (LLPs) have emerged as a compelling signature of physics beyond the standard model, offering unique discovery opportunities at current and future colliders. We present an analysis of charged LLPs leading to signatures with kinked tracks and displaced vertices. Using timing information the search is extended to detector-stable LLPs. We explore the discovery prospects of such particles at the Future Circular Collider~(FCC-ee), a proposed $e^{+}e^{-}$ collider. The clean collision environment of FCC-ee and excellent tracking performance of the IDEA detector enhance the sensitivity to kinked-track signatures, which are considerably more challenging to reconstruct in the high-occupancy environment of hadron colliders. The excellent timing resolution of the timing layer enables us to infer the mass of the detector stable particles. As a benchmark the stau pair production in the gauge mediated supersymmetry breaking (GMSB) within the minimal supersymmetric standard model scenario is considered. In this model the lightest supersymmetric particle is a gravitino and the next-to-lightest supersymmetric particle is the stau, the superpartner of the tau lepton. Discovery sensitivity up to the kinematic limit is obtained for the $ZH$ and $t\bar{t}$ runs of the planned FCC-ee operation. We demonstrate that a potential discovery would allow for a precise $\tilde\tau$ mass measurement.

==> KVDV_NEW.tex <==

% \newpage
\begin{figure}[h]
\centering
\begin{minipage}{0.48\linewidth}
\centering
\begin{tikzpicture}[scale=1.0]
  % --- COLORS ---
  \colorlet{beamcol}{black}
  \colorlet{SVcol}{blue}
  \colorlet{Bccol}{blue}
  \colorlet{IP}{red}
  \colorlet{Jpsicol}{red!90!black}
  \colorlet{taucol}{orange!95!black}
  \colorlet{staucol1}{orange!95!black}
  \colorlet{staucol2}{orange!95!black}
  \colorlet{pioncol}{Jpsicol}
  \colorlet{invcol}{black!50}
  \colorlet{pioncol1}{red!85!black}
  \colorlet{dvcol}{blue!70!black}
  \colorlet{invcol1}{black!50}
  % --- COORDINATES ---
  \coordinate (IP) at (0,0);
  \coordinate (KV)  at (1.1,1.7);
  \coordinate (DV) at (-1.1,-1.7);
  % Beam line
  \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (-4,0) -- (0,0);
  \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (+4,0) -- (0,0);
  \node[beamcol] at ([xshift=-50pt, yshift=-10pt] IP) {$e^+$};
  \node[beamcol] at ([xshift=50pt, yshift=-10pt] IP) {$e^-$};
  \fill[IP,draw=IP,thick] (IP) circle (2.3pt);
  % Stau track -1
\draw[staucol1,very thick,-{Latex[length=8pt, width=4pt]}]
    (IP) -- (DV)
    node[midway, right=4pt, staucol1] {$\tilde{\tau}^{+}$};
  % Stau track -2
  \draw[staucol2,very thick,-{Latex[length=8pt, width=4pt]}]
    (IP) -- (KV)
    node[midway, right=4pt, staucol2] {$\tilde{\tau}^{-}$};
  % Kink vertex
  \fill[SVcol,draw=Bccol,thick] (KV) circle (2.3pt);
  \node[blue!70!black, above =24 pt, right=10 pt] at (KV) {Kinked Track};

  % Charged pion
  \draw[pioncol,line width=1.3pt,-{Latex[length=6pt]}]
    (KV) -- ++(30:3) node[above right=4pt] {$\pi^{-}$};
  % Gravitino
  \draw[invcol,line width=1pt,dashed,-{Latex[length=6pt]}]
    (KV) -- ++(140:2.6) node[above left=1pt] {$\tilde{G}$};
  % Displaced vertex
  \fill[dvcol] (DV) circle (2.3pt);
  \node[dvcol, above left ] at (DV) {Displaced Vertex};
  \draw[pioncol1,line width=1.2pt,-{Latex[length=6pt]}]
    (DV) -- ++(-130:2.6) node[below left] {$\pi^\pm$};
  \draw[pioncol1,line width=1.2pt,-{Latex[length=6pt]}]
    (DV) -- ++(-150:2.9) node[left] {$\pi^\mp$};
  \draw[pioncol1,line width=1.2pt,-{Latex[length=6pt]}]
    (DV) -- ++(-170:2.5) node[above left] {$\pi^\pm$};
  % Invisible gravitino
  \draw[invcol1, line width=1pt,dashed,-{Latex[length=6pt]}]
    (DV) -- ++(-35:2.6) node[below right=1pt] {$\tilde{G}$};
\end{tikzpicture}
\end{minipage}
\caption{Representative signal topology for long-lived $\tilde{\tau}$ pair production. One $\tilde{\tau}$ decays into a charged pion and a gravitino and as the gravitino is invisible, the $\tilde{\tau}$ track appears to be kinked. The other $\tilde{\tau}$ decays to three charged pions, whose tracks can be fitted into a vertex called the displaced vertex.}
\label{fig:KVDV_together}
\end{figure}

% \newpage
% \begin{figure}[h]
% \centering
% \begin{minipage}{0.80\linewidth}
% \centering
% \begin{tikzpicture}[scale=1.0]
%   \colorlet{beamcol}{black}
%   \colorlet{SVcol}{blue}
%   \colorlet{Bccol}{blue}
%   \colorlet{IP}{red}
%   \colorlet{pioncol}{red!90!black}
%   \colorlet{staucol1}{orange!95!black}
%   \colorlet{staucol2}{orange!95!black}
%   \colorlet{invcol}{black!50}
%   \colorlet{pioncol1}{red!85!black}
%   \colorlet{dvcol}{blue!70!black}
%   \colorlet{invcol1}{black!50}
%   \colorlet{timingcol}{green!55!black}

%   \coordinate (IP) at (0,0);

%   % Timing layer rectangle
%   \fill[timingcol!12] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \draw[timingcol, line width=1.8pt] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \node[timingcol, font=\small\bfseries, anchor=south west]
%     at (3.05, 2.4) {Timing Layer};

%   % Beam line
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (-6.2,0) -- (0,0);
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (+6.2,0) -- (0,0);
%   \node[beamcol, anchor=north] at (-5.2,-0.18) {$e^+$};
%   \node[beamcol, anchor=north] at ( 5.2,-0.18) {$e^-$};

%   % IP
%   \fill[IP, draw=IP, thick] (IP) circle (2.3pt);
%   \node[IP, anchor=north east, font=\small] at (-0.12,-0.12) {IP};

%   % -------------------------------------------------------
%   % STAU- (upper right): exits timing layer, decays just outside
%   % KV placed close to but outside the top wall
%   % -------------------------------------------------------
%   % direction ~56 deg; exit top at x=1.62, y=2.4
%   % KV just beyond: continuing same direction a short step
%   \coordinate (TLexit) at (1.62, 2.4);
%   \coordinate (KV) at (2.05, 3.05);  % close to timing layer

%   \draw[staucol2, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (KV)
%     node[midway, right=7pt] {$\tilde{\tau}^{-}$};

%   \fill[timingcol!80!black] (TLexit) circle (3.0pt);
%   \fill[SVcol, draw=Bccol, thick] (KV) circle (2.5pt);

%   % Ghost continuation
%   \draw[staucol2, thin, dashed, opacity=0.35]
%     (KV) -- ++(56:0.7);

%   % Pion from kink
%   \draw[pioncol, line width=1.3pt, -{Latex[length=6pt]}]
%     (KV) -- ++(15:2.8)
%     node[anchor=west] {$\pi^{-}$};

%   % Gravitino from kink
%   \draw[invcol, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (KV) -- ++(100:2.0)
%     node[anchor=south] {$\tilde{G}$};

%   % -------------------------------------------------------
%   % STAU+ (lower left): decays INSIDE timing layer at DV
%   % DV placed clearly inside the rectangle
%   % -------------------------------------------------------
%   \coordinate (DV) at (-1.5, -1.5);  % inside the box

%   \draw[staucol1, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (DV)
%     node[midway, left=7pt] {$\tilde{\tau}^{+}$};

%   % No hit marker needed — never exits
%   \fill[dvcol] (DV) circle (2.5pt);

%   % Three pions from DV
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-70:2.5)  node[anchor=north]      {$\pi^\pm$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-120:2.0) node[anchor=north east] {$\pi^\mp$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-160:1.8) node[anchor=east]       {$\pi^\pm$};

%   % Gravitino from DV
%   \draw[invcol1, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (DV) -- ++(-30:2.8)
%     node[anchor=north west] {$\tilde{G}$};

% \end{tikzpicture}
% \end{minipage}
% \caption{Signal topology where one $\tilde{\tau}^{-}$ decays just outside the timing layer into a $\pi^{-}$ and $\tilde{G}$, producing a kinked track, while the $\tilde{\tau}^{+}$ decays inside the timing layer into three charged pions and $\tilde{G}$, reconstructing a displaced vertex within the tracker volume.}
% \label{fig:one_inside_one_outside}
% \end{figure}

% \newpage
% \begin{figure}[h]
% \centering
% \begin{minipage}{0.80\linewidth}
% \centering
% \begin{tikzpicture}[scale=1.0]
%   \colorlet{beamcol}{black}
%   \colorlet{SVcol}{blue}
%   \colorlet{Bccol}{blue}
%   \colorlet{IP}{red}
%   \colorlet{pioncol}{red!90!black}
%   \colorlet{staucol1}{orange!95!black}
%   \colorlet{staucol2}{orange!95!black}
%   \colorlet{invcol}{black!50}
%   \colorlet{pioncol1}{red!85!black}
%   \colorlet{dvcol}{blue!70!black}
%   \colorlet{invcol1}{black!50}
%   \colorlet{timingcol}{green!55!black}

%   \coordinate (IP) at (0,0);

%   % Timing layer rectangle
%   \fill[timingcol!12] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \draw[timingcol, line width=1.8pt] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \node[timingcol, font=\small\bfseries, anchor=south west]
%     at (3.05, 2.4) {Timing Layer};

%   % Beam line
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (-6.2,0) -- (0,0);
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (+6.2,0) -- (0,0);
%   \node[beamcol, anchor=north] at (-5.2,-0.18) {$e^+$};
%   \node[beamcol, anchor=north] at ( 5.2,-0.18) {$e^-$};

%   % IP
%   \fill[IP, draw=IP, thick] (IP) circle (2.3pt);
%   \node[IP, anchor=north east, font=\small] at (-0.12,-0.12) {IP};

%   % -------------------------------------------------------
%   % STAU- (upper right): exits top wall, decays just outside as KV
%   % -------------------------------------------------------
%   \coordinate (TLexit) at (1.62, 2.4);
%   \coordinate (KV) at (2.05, 3.05);

%   \draw[staucol2, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (KV)
%     node[midway, right=7pt] {$\tilde{\tau}^{-}$};

%   \fill[timingcol!80!black] (TLexit) circle (3.0pt);
%   \fill[SVcol, draw=Bccol, thick] (KV) circle (2.5pt);

%   \draw[staucol2, thin, dashed, opacity=0.35]
%     (KV) -- ++(56:0.7);

%   \draw[pioncol, line width=1.3pt, -{Latex[length=6pt]}]
%     (KV) -- ++(15:2.8)
%     node[anchor=west] {$\pi^{-}$};

%   \draw[invcol, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (KV) -- ++(100:2.0)
%     node[anchor=south] {$\tilde{G}$};

%   % -------------------------------------------------------
%   % STAU+ (lower left): exits bottom wall, decays just outside as DV
%   % -------------------------------------------------------
%   % direction toward lower-left ~225 deg; exit bottom at y=-2.4
%   % pick angle ~-124 deg (lower-left); exit bottom: 
%   % x at y=-2.4 with slope tan(-124 deg): x = -2.4/tan(56) ~ -1.62
%   \coordinate (TLexit2) at (-1.62, -2.4);
%   \coordinate (DV) at (-2.05, -3.05);   % mirror of KV

%   \draw[staucol1, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (DV)
%     node[midway, left=7pt] {$\tilde{\tau}^{+}$};

%   \fill[timingcol!80!black] (TLexit2) circle (3.0pt);
%   \fill[dvcol] (DV) circle (2.5pt);

%   % Three pions from DV, sent downward/leftward
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-80:2.2)  node[anchor=north]      {$\pi^\pm$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-130:2.0) node[anchor=north east] {$\pi^\mp$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-165:1.9) node[anchor=east]       {$\pi^\pm$};

%   % Gravitino from DV
%   \draw[invcol1, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (DV) -- ++(-20:2.8)
%     node[anchor=north west] {$\tilde{G}$};

% \end{tikzpicture}
% \end{minipage}
% \caption{Signal topology where both $\tilde{\tau}$ tracks cross the timing layer (green dots mark the hits) before decaying. The $\tilde{\tau}^{-}$ decays just outside into a $\pi^{-}$ and $\tilde{G}$, producing a kinked track. The $\tilde{\tau}^{+}$ decays just outside into three charged pions and $\tilde{G}$, reconstructing a displaced vertex beyond the timing layer.}
% \label{fig:both_outside}
% \end{figure}

% \newpage
% \begin{figure}[h]
% \centering
% \begin{minipage}{0.80\linewidth}
% \centering
% \begin{tikzpicture}[scale=1.0]
%   \colorlet{beamcol}{black}
%   \colorlet{SVcol}{blue}
%   \colorlet{Bccol}{blue}
%   \colorlet{IP}{red}
%   \colorlet{pioncol}{red!90!black}
%   \colorlet{staucol1}{orange!95!black}
%   \colorlet{staucol2}{orange!95!black}
%   \colorlet{invcol}{black!50}
%   \colorlet{pioncol1}{red!85!black}
%   \colorlet{dvcol}{blue!70!black}
%   \colorlet{invcol1}{black!50}
%   \colorlet{timingcol}{green!55!black}

%   \coordinate (IP) at (0,0);

%   % Timing layer rectangle
%   \fill[timingcol!12] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \draw[timingcol, line width=1.8pt] (-3.0,-2.4) rectangle (3.0, 2.4);
%   \node[timingcol, font=\small\bfseries, anchor=south west]
%     at (3.05, 2.4) {Timing Layer};

%   % Beam line
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (-6.2,0) -- (0,0);
%   \draw[beamcol, very thick, dashed, -{Latex[length=8pt]}] (+6.2,0) -- (0,0);
%   \node[beamcol, anchor=north] at (-5.2,-0.18) {$e^+$};
%   \node[beamcol, anchor=north] at ( 5.2,-0.18) {$e^-$};

%   % IP
%   \fill[IP, draw=IP, thick] (IP) circle (2.3pt);
%   \node[IP, anchor=north east, font=\small] at (-0.12,-0.12) {IP};

%   % -------------------------------------------------------
%   % STAU- (upper right): exits top wall, decays just outside
%   % -------------------------------------------------------
%   \coordinate (TLexit) at (1.62, 2.4);
%   \coordinate (KV) at (2.05, 3.05);

%   % Stau track with beta label at the midpoint
%   \draw[staucol2, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (KV);
%   \node[staucol2, anchor=west, font=\small]
%     at (0.85, 1.1) {$\tilde{\tau}^{-}$};
%   \node[staucol2, anchor=west, font=\small]
%     at (0.55, 0.55) {$(\beta < 1)$};

%   % TOF hit on timing layer
%   \fill[timingcol!80!black] (TLexit) circle (3.5pt);
%   % TOF label with arrow, placed to upper-right of hit to avoid stau track
%   \draw[timingcol!70!black, thin, -{Latex[length=4pt]}]
%     (2.55, 3.15) -- (1.75, 2.52);
%   \node[timingcol!70!black, font=\scriptsize, anchor=west, align=left]
%     at (2.58, 3.15) {TOF hit\\$t_{\tilde{\tau}^{-}}$};

%   % KV dot
%   \fill[SVcol, draw=Bccol, thick] (KV) circle (2.5pt);

%   % Ghost stau continuation
%   \draw[staucol2, thin, dashed, opacity=0.35]
%     (KV) -- ++(56:0.7);

%   % Pion from kink
%   \draw[pioncol, line width=1.3pt, -{Latex[length=6pt]}]
%     (KV) -- ++(15:2.8)
%     node[anchor=west] {$\pi^{-}$};

%   % Gravitino from kink
%   \draw[invcol, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (KV) -- ++(100:2.0)
%     node[anchor=south] {$\tilde{G}$};

%   % -------------------------------------------------------
%   % STAU+ (lower left): decays INSIDE timing layer
%   % -------------------------------------------------------
%   \coordinate (DV) at (-1.5, -1.5);

%   \draw[staucol1, very thick, -{Latex[length=8pt, width=4pt]}]
%     (IP) -- (DV);
%   \node[staucol1, anchor=east, font=\small]
%     at (-0.65, -0.75) {$\tilde{\tau}^{+}$};
%   \node[staucol1, anchor=east, font=\small]
%     at (-0.40, -1.25) {$(\beta < 1)$};

%   % DV dot (no TOF hit — never exits timing layer)
%   \fill[dvcol] (DV) circle (2.5pt);

%   % Three pions from DV
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-70:2.5)  node[anchor=north]      {$\pi^\pm$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-120:2.0) node[anchor=north east] {$\pi^\mp$};
%   \draw[pioncol1, line width=1.2pt, -{Latex[length=6pt]}]
%     (DV) -- ++(-160:1.8) node[anchor=east]       {$\pi^\pm$};

%   % Gravitino from DV
%   \draw[invcol1, line width=1pt, dashed, -{Latex[length=6pt]}]
%     (DV) -- ++(-25:3.0)
%     node[anchor=north west] {$\tilde{G}$};

%   % Note: no TOF hit for stau+ since it decays inside
%   \node[timingcol!70!black, font=\scriptsize, align=center]
%     at (-2.2, 0.9) {No TOF hit\\($\tilde{\tau}^{+}$ decays\\inside)};

% \end{tikzpicture}
% \end{minipage}
% \caption{Signal topology where the $\tilde{\tau}^{-}$ ($\beta < 1$) crosses the timing layer, registering a delayed TOF hit $t_{\tilde{\tau}^{-}}$, before decaying just outside into a $\pi^{-}$ and invisible $\tilde{G}$, producing a kinked track. The $\tilde{\tau}^{+}$ ($\beta < 1$) decays inside the timing layer into three charged pions and $\tilde{G}$, leaving no TOF hit.}
% \label{fig:one_inside_one_outside}
% \end{figure}

% \newpage


==> current_results.tex <==

\begin{table}[H] 
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{|l||c|c|c|c|c|c|c|c|} \hline
         & stau 20\cm & stau 1.5\,m & stau 3\,m & WW & ZZ & ZH_{H\to bb} & $\nu_e \nu_e H_{H\to\tau\tau}$ & $bbH_{H\to\tau\tau}$ \\ \hline
         
        selNone & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
        semiLepHad & 0.873 & 0.898 & 0.909 & 0.897 & 0.755 & 0.722 & 0.887 & 0.61 \\
        semiLeptonic & 0.401 & 0.422 & 0.408 & 0.416 & 0.197 & 0.368 & 0.438 & 0.389 \\
        semiLeptonic_KV & 0.000564 & 0.144 & 0.159 & 0.00171 & 0.00105 & 0.0002 & 0. & 0. \\
        semiLep_DV & 0.0608 & 0.0296 & 0.0237 & 0.0853 & 0.122 & 0.329 & 0.0727 & 0.337 \\
        hadronic & 0.472 & 0.476 & 0.502 & 0.481 & 0.558 & 0.354 & 0.449 & 0.221 \\
        hadronic_none & 0.346 & 0.259 & 0.272 & 0.341 & 0.377 & 0.037 & 0.32 & 0.0265 \\
        hadronic_short_KV & 0.000677 & 0.15 & 0.17 & 0.00323 & 0.0044 & 0.0009 & 0. & 0.0001 \\
        hadronic_short_DV & 0.125 & 0.0669 & 0.0597 & 0.138 & 0.176 & 0.316 & 0.129 & 0.195 \\
        hadronic_KV & 0.000677 & 0.15 & 0.17 & 0.00323 & 0.0044 & 0.0009 & 0. & 0.0001 \\
        hadronic_DV & 0.125 & 0.0669 & 0.0597 & 0.138 & 0.176 & 0.316 & 0.129 & 0.195 \\
        hadronic_allchannels & 0.126 & 0.204 & 0.212 & 0.14 & 0.18 & 0.316 & 0.129 & 0.195 \\
        \hline
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{table}

ADDED NO RECO LEPTON IN DV REGION (hadronic) and one reco lepton only in semilep:
\begin{table}[H] 
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{|l||c|c|c|c|c|c|c|c|} \hline
         &   stau 20\,cm & stau 1.5\,m & stau 3\,m & WW & ZZ & ZH_{H\to bb} & $\nu_e \nu_e H_{H\to\tau\tau}$ & $bbH_{H\to\tau\tau}$ \\
        selNone & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
        semiLeptonic & 0.46 & 0.475 & 0.454 & 0.467 & 0.385 & 0.506 & 0.497 & 0.555 \\
        \rowcolor{green!15} semiLeptonic\_KV & \sout{0.000677} & 0.164 & 0.18 & 0.00171 & 0.0022 & 0.0003 & 0. & 0. \\
        \rowcolor{green!15} semiLep\_DV & \textbf{0.0608} & 0.0296 & 0.0237 & 0.0853 & 0.122 & 0.329 & 0.0727 & 0.337 \\
        % hadronic\_short\_KV & {0.00169} & 0.333 & 0.369 & 0.00524 & 0.0067 & 0.0012 & 0. & 0.0001 \\
        \rowcolor{blue!15} hadronic\_DV & \textbf{0.125} & 0.0669 & 0.0597 & 0.138 & 0.176 & 0.316 & 0.129 & 0.195 \\
        \rowcolor{red!15} hadronic\_KV & \sout{0.00169} & 0.333 & 0.369 & 0.00524 & 0.0067 & 0.0012 & 0. & 0.0001 \\
        % hadronic\_DV & 0.125 & 0.0669 & 0.0597 & 0.138 & 0.176 & 0.316 & 0.129 & 0.195 \\
        \hline
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}[H]
    \centering
    \begin{tabular}{|l|p{10cm}|}
        \hline
        Selection & Cut Description \\ \hline\hline
        selNone & No selection: all events with any number of reconstructed tracks. \\ \hline
        semiLepHad & Require 0 or 1 reconstructed leptons (electron or muon). Keeps events with exactly 1 electron or 1 muon, or zero leptons. \\ \hline
        semiLeptonic & Require exactly 1 reconstructed lepton (electron or muon). \\ \hline
        \rowcolor{green!15} semiLeptonic\_KV & Same as semiLeptonic, but also remove events with 2 or more kink candidates (nKinkCandidates\_passVeto < 2). \\ \hline
        \rowcolor{green!15} semiLep\_KVDV & One reconstructed lepton + either 1 kink vertex or 1 displaced vertex (DV) + less than 4 jets. \\ \hline
        hadronic & Require 0 reconstructed leptons (electron = 0, muon = 0). \\ \hline
        \rowcolor{blue!15} hadronic\_small\_DV & Hadronic events with at least one DV and fewer than 2 kink candidates. Designed for small $\beta\gamma c\tau$ scenarios. \\ \hline
        \rowcolor{blue!15} hadronic\_small\_1prong & Hadronic events with small $\beta\gamma c\tau$, both taus decaying to 1-prong, some visible energy. also require less than 2 DV and NO kinked vertices. \\ \hline
        \rowcolor{red!15} hadronic\_KV & Hadronic events with fewer than 3 kink candidates but at least one (large $\beta\gamma c\tau$). \\ \hline
        \rowcolor{red!15} hadronic\_KVDV & Hadronic events with fewer than 4 jets, fewer than 3 kink candidates but atleast one, and combinations of kink/DV satisfying one of three conditions. Targets large $\beta\gamma c\tau$ scenarios with DVs or kinks. \\ \hline
    \end{tabular}
    \caption{Summary of selection cuts used in the analysis, color-coded according to final-state type. Green = semi-leptonic, Blue = hadronic small DV/1-prong, Red = hadronic KV/KVDV.}
    \label{tab:cuts_colored}
\end{table}


Yields:
\begin{table}[H]
    \resizebox{\textwidth}{!}{
        \begin{tabular}{|l||c|c|c|c|c|c|c|c|} \hline
         & All events & selNone & semiLeptonic_KV & semiLep_DV & hadronic KV & hadronic_DV  \\ \hline

         \rowcolor{red!15}  FCCee_105_stau_20cm_ctau_ecm_240 & 4.95e+05 $\pm$ 1.67e+03 & 4.95e+05 $\pm$ 1.67e+03 & 2.04e+03 $\pm$ 1.07e+02 & 2.93e+04 $\pm$ 4.05e+02 & 5.45e+04 $\pm$ 5.53e+02 & 4.09e+03 $\pm$ 1.52e+02 \\

        \rowcolor{red!15}  FCCee_115_stau_20cm_ctau_ecm_240 & 1.01e+05 $\pm$ 3.42e+02 & 1.01e+05 $\pm$ 3.42e+02 & 4.61e+00 $\pm$ 2.30e+00 & 5.59e+03 $\pm$ 8.03e+01 & 9.85e+03 $\pm$ 1.07e+02 & 9.22e+00 $\pm$ 3.26e+00 \\

        FCCee_105_stau_50cm_ctau_ecm_240 & 5.17e+05 $\pm$ 1.70e+03 & 5.17e+05 $\pm$ 1.70e+03 & 3.41e+04 $\pm$ 4.37e+02 & 2.61e+04 $\pm$ 3.83e+02 & 4.93e+04 $\pm$ 5.26e+02 & 6.77e+04 $\pm$ 6.17e+02 \\

        FCCee_115_stau_50cm_ctau_ecm_240 & 1.03e+05 $\pm$ 3.44e+02 & 1.03e+05 $\pm$ 3.44e+02 & 1.41e+03 $\pm$ 4.03e+01 & 5.43e+03 $\pm$ 7.91e+01 & 9.56e+03 $\pm$ 1.05e+02 & 2.70e+03 $\pm$ 5.58e+01 \\

        \rowcolor{blue!15} FCCee_105_stau_1m_ctau_ecm_240 & 5.34e+05 $\pm$ 5.47e+03 & 5.34e+05 $\pm$ 5.47e+03 & 0. & 3.14e+04 $\pm$ 1.33e+03 & 4.89e+04 $\pm$ 1.66e+03 & 0. \\


        \rowcolor{red!15}  FCCee_105_stau_2m_ctau_ecm_240 & 5.48e+05 $\pm$ 1.75e+03 & 5.48e+05 $\pm$ 1.75e+03 & 9.78e+04 $\pm$ 7.41e+02 & 1.14e+04 $\pm$ 2.53e+02 & 3.13e+04 $\pm$ 4.19e+02 & 2.08e+05 $\pm$ 1.08e+03 \\

        \rowcolor{red!15}  FCCee_115_stau_2m_ctau_ecm_240 & 1.11e+05 $\pm$ 3.57e+02 & 1.11e+05 $\pm$ 3.57e+02 & 1.76e+04 $\pm$ 1.42e+02 & 3.42e+03 $\pm$ 6.28e+01 & 6.90e+03 $\pm$ 8.92e+01 & 3.43e+04 $\pm$ 1.99e+02 \\
 

        FCCee_105_stau_4m_ctau_ecm_240 & 5.52e+05 $\pm$ 1.76e+03 & 5.52e+05 $\pm$ 1.76e+03 & 7.69e+04 $\pm$ 6.57e+02 & 5.31e+03 $\pm$ 1.73e+02 & 2.35e+04 $\pm$ 3.63e+02 & 1.78e+05 $\pm$ 9.99e+02 \\
        FCCee_110_stau_4m_ctau_ecm_240 & 3.10e+05 $\pm$ 9.89e+02 & 3.10e+05 $\pm$ 9.89e+02 & 4.83e+04 $\pm$ 3.90e+02 & 3.66e+03 $\pm$ 1.08e+02 & 1.41e+04 $\pm$ 2.11e+02 & 1.07e+05 $\pm$ 5.82e+02 \\

        p8_ee_WW_ecm240 & 1.76e+08 $\pm$ 1.25e+06 & 1.76e+08 $\pm$ 1.25e+06 & 0. & 1.53e+07 $\pm$ 3.68e+05 & 2.48e+07 $\pm$ 4.69e+05 & 0. \\
        p8_ee_ZZ_ecm240 & 1.41e+07 $\pm$ 1.86e+05 & 1.41e+07 $\pm$ 1.86e+05 & 0. & 1.40e+06 $\pm$ 5.85e+04 & 2.18e+06 $\pm$ 7.30e+04 & 0. \\
        mgp8_ee_zh_ecm240_hbb & 1.08e+07 $\pm$ 1.08e+05 & 1.08e+07 $\pm$ 1.08e+05 & 0. & 2.40e+06 $\pm$ 5.10e+04 & 2.38e+06 $\pm$ 5.07e+04 & 0. \\
        wzp6_ee_nuenueH_Htautau_ecm240 & 1.18e+04 $\pm$ 1.14e+02 & 1.18e+04 $\pm$ 1.14e+02 & 0. & 8.50e+02 $\pm$ 3.05e+01 & 1.52e+03 $\pm$ 4.09e+01 & 0. \\
        wzp6_ee_bbH_Htautau_ecm240 & 2.03e+04 $\pm$ 3.21e+02 & 2.03e+04 $\pm$ 3.21e+02 & 0. & 5.19e+03 $\pm$ 1.62e+02 & 2.97e+03 $\pm$ 1.23e+02 & 0. \\
        \hline
    \end{tabular}}
    \caption{Caption}
    \label{tab:eff_tb}
\end{table}


==> limits.tex <==
\begin{figure}[H]
\centering

% Row 1: 0.5 m, 1 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_0.5m.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_1m.png}
\end{minipage}

\vspace{0.4cm}

% Row 2: 5 m, 10 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_5m.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_10m.png}
\end{minipage}

\vspace{0.4cm}

% Row 3: 20 m, 50 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_20m.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_240GeV_2109/brazil_plot_lifetime_all_channels_50m.png}
\end{minipage}

\caption{Expected 95\% CL limits on the stau production cross section as a function of the stau mass for different proper lifetimes ($c\tau = 0.5$~m, 1~m, 5~m, 10~m, 20~m and 50~m). The results correspond to the full FCC-ee runtime at $\sqrt{s}=240$~GeV, assuming an integrated luminosity of $2.7~\mathrm{ab}^{-1}$.}
\label{fig:brazil_plots_3years}

\end{figure}

==> limits_365.tex <==
\begin{figure}[H]
\centering

% Row 1: 0.5 m, 1 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_0.5m_2109.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_1m_2109.png}
\end{minipage}

\vspace{0.4cm}

% Row 2: 5 m, 10 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_5m_2109.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_10m_2109.png}
\end{minipage}

\vspace{0.4cm}

% Row 3: 20 m, 50 m
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_20m_2109.png}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{plots_365GeV_2109/brazil_plot_lifetime_all_channels_50m_2109.png}
\end{minipage}

\caption{Expected 95\% CL limits on the stau production cross section as a function of the stau mass for different proper lifetimes ($c\tau = 0.5$~m, 1~m, 5~m, 10~m, 20~m and 50~m). The results correspond to the full FCC-ee runtime at $\sqrt{s}=365$~GeV, assuming an integrated luminosity of $0.67~\mathrm{ab}^{-1}$.}
\label{fig:brazil_plots_3years_365}

\end{figure}

==> signal_feynmann.tex <==
% \begin{figure}[ht]
% \centering
% \begin{minipage}{0.48\textwidth}
% \centering
% \begin{tikzpicture}[scale=0.8]
% \tikzset{every label/.append style={font=\small}}

%     \begin{feynman}
%       % Proton-proton collision vertex
%       \vertex (v1) at (-2.75,  0);
%       \fill[pattern=vertical lines, pattern color=green!40!black, opacity=1.5] (v1) circle (0.3);
      
%       % Stau production
%       \vertex (f1) at (-0.5,  1.5);
%       \vertex (f2) at (-0.5, -1.5);

%       \vertex (t1) at (1.5,  2.5);
%       \node[above left] at (t1) {\small$\tau^{-}$};
%       \vertex (n1_1) at (1.5,  0.5) {\small${\tilde{G}}$};
 
%       \vertex (W1) at (3.5, 3.25);
%       \node[above left] at (W1) {\small$W^{-}$};
%       \vertex (nu_tau) at (3.5, 1.75) {\small$\nu_\tau$};

%       \vertex (muon) at (5.25, 4.25){\small$\mu$/$e^{-}$};
%       \vertex (nu_mu) at (5.25, 2.25) {\small$\bar\nu_\mu$/$\bar\nu_{e}$};
      
%       % Hadronic tau decay (jet formation)
%       \vertex (t2) at (1.5, -2.5);
%       \node[below left] at (t2) {\small$\tau^{+}$};
%       \vertex (n2) at (1.5, -0.5) {\small ${\tilde{G}}$};

%       % tau neutrino from hadronic tau+ decay
%       \vertex (nu_tau2) at (3.0, -1.5) {\small$\bar\nu_\tau$};

%       \vertex (wboson2) at (3.20, -3.2);
%       \node[below left] at (wboson2) {\small$W^{+}$};
      
%       \vertex (pion1) at (5.95 ,-4.0){\small$\pi^{0}$};
%       \vertex (pion2) at (5.95 ,-3.4){\small$\pi^{0}$};
%       \vertex (pion3) at (5.95 ,-2.7){\small$\pi^{+}$};

%       % Tau decaying hadronically and forming a jet
%       \coordinate (jetStart) at (3.5, -3.2);
%       \draw[decorate, decoration={snake, amplitude=0.2mm, segment length=2mm}] (wboson2) -- (jetStart);
      
%       % Define and draw the colored cone for the jet
%       \tikzset{mycone/.pic={
%         \draw[blue!50!black, very thin] (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%         \shade[left color=blue!10!white, right color=blue!60!black, opacity=0.4]
%           (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%       }}
      
%       \pic at (jetStart) {mycone};
      
%       % Feynman diagram connections
%       \diagram*{
%         (v1) -- [scalar, edge label=\small$\tilde{\tau}^{-}$] (f1),
%         (v1) -- [scalar, edge label=\small$\tilde{\tau}^{+}$] (f2),

%         (f1) -- [fermion] (t1),
%         (f1) -- [boson] (n1_1),

%         (t1) -- [boson] (W1),
%         (t1) -- [fermion] (nu_tau),

%         (W1) -- [fermion] (muon),
%         (W1) -- [fermion] (nu_mu),

%         % tau+ decays to anti-nu_tau + W+
%         (f2) -- [fermion] (t2),
%         (f2) -- [boson] (n2),
%         (t2) -- [fermion] (nu_tau2),
%         (t2) -- [boson] (wboson2),

%         (jetStart) -- [fermion] (pion1),
%         (jetStart) -- [fermion] (pion2),
%         (jetStart) -- [fermion] (pion3),
%       };
%     \end{feynman}
% \end{tikzpicture}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \begin{tikzpicture}[scale=0.8]
% \tikzset{every label/.append style={font=\small}}

%     \begin{feynman}
%       % Proton-proton collision vertex
%       \vertex (v1) at (-2,  0);
%       \fill[pattern=vertical lines, pattern color=green!40!black, opacity=1] (v1) circle (0.3);
      
%       % Stau production
%       \vertex (f1) at (0,  1.5);
%       \vertex (f2) at (0, -1.5);

%       \vertex (t1) at (2,  2);
%       \node[above left] at (t1) {\small$\tau^{+}$};
%       \vertex (n1_1) at (2,  0.5) {\small${\tilde{G}}$};

%       % tau+ -> anti-nu_tau + W+
%       \vertex (nu_tau_top) at (3.5,  0.9) {\small$\bar\nu_\tau$};
%       \vertex (W111) at (3.5,  2.8);
%       \node[above left] at (W111) {\small$W^{+}$};

%       \vertex (pion4) at (5.95 ,3.5) {\small$\pi^{0}$};
%       \vertex (pion5) at (5.95 ,2.9) {\small$\pi^{0}$};
%       \vertex (pion6) at (5.95 ,2.3) {\small$\pi^{+}$};

%       % tau- -> nu_tau + W-
%       \vertex (t2) at (2, -2);
%       \node[below left] at (t2) {\small$\tau^{-}$};
%       \vertex (n2) at (2, -0.5){\small${\tilde{G}}$};

%       \vertex (nu_tau_bot) at (3.5, -0.9) {\small$\nu_\tau$};
%       \vertex (W222) at (3.5,  -2.8);
%       \node[below left] at (W222) {\small$W^{-}$};

%       \vertex (pion1) at (5.95 ,-3.3) {\small$\pi^{-}$};
%       \vertex (pion2) at (5.95 ,-2.7) {\small$\pi^{+}$};
%       \vertex (pion3) at (5.95 ,-2.1) {\small$\pi^{-}$};
      
%       % Hadronic tau- decay jet
%       \coordinate (jetStart) at (3.5, -2.8);
%       \draw[decorate, decoration={snake, amplitude=0.2mm, segment length=2mm}] (W222) -- (jetStart);
      
%       \tikzset{mycone/.pic={
%         \draw[blue!50!black, very thin] (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%         \shade[left color=blue!10!white, right color=blue!60!black, opacity=0.4]
%           (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%       }}
      
%       \pic at (jetStart) {mycone};

%       % Hadronic tau+ decay jet
%       \coordinate (jetStart1) at (3.5, 2.8);
%       \draw[decorate, decoration={snake, amplitude=0.2mm, segment length=2mm}] (W111) -- (jetStart1);
      
%       \tikzset{mycone1/.pic={
%         \draw[blue!50!black, very thin] (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%         \shade[left color=blue!10!white, right color=blue!60!black, opacity=0.4]
%           (0,0) -- (1.5,0.7) arc(27:-27:1.6) -- cycle;
%       }}
      
%       \pic at (jetStart1) {mycone1};
      
%       % Feynman diagram connections
%       \diagram*{
%         (v1) -- [scalar, edge label=\small$\tilde{\tau}^{+}$] (f1),
%         (v1) -- [scalar, edge label=\small$\tilde{\tau}^{-}$] (f2),

%         (f1) -- [fermion] (t1),
%         (f1) -- [boson] (n1_1),

%         % tau+ -> anti-nu_tau + W+
%         (t1) -- [fermion] (nu_tau_top),
%         (t1) -- [boson] (W111),

%         (f2) -- [fermion] (t2),
%         (f2) -- [boson] (n2),

%         % tau- -> nu_tau + W-
%         (t2) -- [fermion] (nu_tau_bot),
%         (t2) -- [boson] (W222),

%         (jetStart) -- [fermion] (pion1),
%         (jetStart) -- [fermion] (pion2),
%         (jetStart) -- [fermion] (pion3),

%         (jetStart1) -- [fermion] (pion4),
%         (jetStart1) -- [fermion] (pion5),
%         (jetStart1) -- [fermion] (pion6),
%       };
%     \end{feynman}
% \end{tikzpicture}
% \end{minipage}

% \caption{Representative decay topologies of $\tilde{\tau}^+\tilde{\tau}^-$ signal events. Left: semileptonic final state, where one $\tau$ decays leptonically ($\tau \to \ell \nu_\ell \nu_\tau$ with $\ell = e,\mu$) and the other decays hadronically ($\tau^+ \to \bar\nu_\tau + W^{+*} \to \bar\nu_\tau + \text{hadrons}$). Right: fully hadronic final state, where both $\tau$ leptons decay hadronically, yielding two hadronic $\tau$ jets. In both cases, additional missing momentum arises from neutrinos and gravitinos ($\tilde{G}$) in the final state.}
% \label{fig:signal_channels}

% \end{figure}






==> theory_motivation.tex <==

\section{Theoretical Motivation}
Supersymmetry (SUSY) is a spacetime symmetry between fermions and bosons, suggesting a superpartner exists for each particle with a spin that differs by exactly half a unit. Despite extensive searches for SUSY particles at the LHC, none have been observed so far. In this paper, we focus on the minimal supersymmetric standard model (MSSM), which is the simplest supersymmetric extension of SM that introduces the minimal particle content required for consistency with supersymmetry, assuming R-parity conservation\footnote{R-parity is defined as \( R = (-1)^{3(B-L)+2s} \), where \( B \) is baryon number, \( L \) is lepton number, and \( s \) is the particle's spin. Standard Model particles have \( R = +1 \) and their superpartners have \( R = -1 \).}. Two of the main mechanisms that can lead to a long-lived stau are discussed in the next section. In the compressed MSSM scenario, the stau acquires a long lifetime due to the small mass difference between it and the LSP. Whereas in GMSB the stau is long-lived due to the weak coupling between it and the gravitino~\cite{GMSB_basic,GMSBllp}.
%Therefore, it is assumed that SUSY is broken in a hidden sector and is mediated to the visible sector through mechanisms such as gravity or gauge mediation. These breaking mechanisms would introduce many new particles and parameters, making the full SUSY model highly complex. To make meaningful and manageable predictions, simplified models are used.


%MSSM introduces two Higgs doublets, resulting in five physical Higgs bosons: two CP-even neutral, one CP-odd neutral, and two charged Higgs bosons. 

\subsection{Compressed MSSM} %%%% NEED TO RECHECK LINE 70

 The mixing of charged and neutral gauginos with the Higgs superpartners (Higgsinos) leads to the formation of new mass eigenstates called charginos (charged) and neutralinos (neutral).  The lightest neutralino ($\chi^{0}_{1}$) is a strong contender to be the lightest SUSY particle (LSP) and for it to be stable and a dark matter candidate, the next-to-lightest supersymmetric particle (NLSP) has to be nearly mass-degenerate with the LSP~\cite{japan_gmsb}. This suppresses the available phase space for its decay and results in a macroscopic lifetime of the NLSP. Various particles can be considered the NLSP, as discussed in Ref.~\cite{fermilab_gmsb}. The stau is taken as the NLSP in this study. This implies all other SUSY decays in the MSSM cascade to the stau, which is a mass eigenstate of the superpartners of the left and right-handed tau leptons:
\begin{equation}
\tilde{\tau} = \cos\theta_\tau \, \tilde{\tau}_L + \sin\theta_\tau \, e^{-i\gamma_\tau} \, \tilde{\tau}_R,
\end{equation}
where $\theta_\tau$ is the stau mixing angle and $\gamma_\tau$ is the CP-violating phase between the left- and right-handed components. In this work, we focus on the mostly right-handed stau scenario ($\theta_\tau \approx \pi/2$) and set $\gamma_\tau = 0$, corresponding to a real mixing without CP violation.

A small mass difference between the stau and the neutralino:

\begin{equation}
\delta m = m_{\tilde{\tau}} - m_{\tilde{\chi}^0_1} 
\end{equation}

suppresses the phase space for decays, resulting in macroscopic stau lifetimes.
The dominant decay modes depend on the value of $\delta m$. For $\delta m > m_\tau$, the stau primarily undergoes the two-body decay $\tilde{\tau} \to \tilde{\chi}_1^0 \tau$. When $m_\pi < \delta m < m_\tau$, two-body decays are kinematically forbidden and three-body decays involving pions become dominant. For even smaller mass splittings ($\delta m < m_\pi$), the stau decays through four-body channels involving leptons and neutrinos. The corresponding decay widths for these processes have been computed in Ref.~\cite{japan_gmsb}.

Near the kinematic threshold, the decay width becomes strongly suppressed. In particular, for small $\delta m$ the three-body decay width approximately scales as
\begin{equation}
\Gamma \propto \delta m^5 ,
\end{equation}
and the stau lifetime is given by
\begin{equation}
\tau = \frac{\hbar}{c~\Gamma}.
\end{equation}
As a result, sufficiently small mass splittings can lead to staus with macroscopic decay lengths that may appear detector-stable. While compressed MSSM scenarios can produce long-lived staus, their parameter space is highly constrained as there is a rapid transition in the stau appearing as either prompt or detector stable. 

%Although the mechanism that gives the stau a long lifetime differs between the neutralino LSP and gravitino LSP scenarios, in practice the resulting long-lived stau states are very similar.

\subsection{GMSB Scenario}
Alternatively, if the gravitino is the LSP, the NLSP has a naturally long lifetime due to its very weak coupling to the gravitino~\cite{japan_gmsb}. Thus the GMSB model predicts stau NLSPs with lifetimes spanning a wide range, from prompt decays to detector-stable charged tracks, depending on the SUSY-breaking scale. This broad lifetime range makes the GMSB stau scenario particularly well suited for sensitivity studies at FCC-ee, where clean experimental conditions allow precise reconstruction of displaced or metastable charged particles. In Gauge Mediated Supersymmetry Breaking models, supersymmetry breaking occurs in a hidden sector and is transmitted to the MSSM fields through gauge interactions via messenger particles~\cite{GMSBllp}. As a consequence of this mediation mechanism, the gravitino becomes the lightest supersymmetric particle (LSP) and typically has a very small mass in the eV--keV range. 

Depending on the model parameters, several candidates can arise as the next-to-lightest supersymmetric particle (NLSP)~\cite{fermilab_gmsb}. In this work we consider the scenario where the lighter stau $\tilde{\tau}$ is the NLSP. In GMSB models with conserved R-parity, the stau NLSP decays predominantly via:

\begin{equation}
\tilde{\tau}\to \tau \, \tilde{G}.
\label{equation:staudecay}
\end{equation}

The coupling is suppressed by the supersymmetry breaking scale \cite{fermilab_gmsb}:
\begin{equation}
\tau =
\frac{1}{k^{2}}
\left( \frac{100~\mathrm{GeV}}{m_{\mathrm{\tilde\tau}}} \right)^{5}
\left( \frac{\sqrt{F}}{100~\mathrm{TeV}} \right)^{4}
\times 3 \times 10^{-13}\ \mathrm{s} ,
\end{equation}

where the $\tau$ refers to the lifetime of the stau, $F$ is the SUSY breaking scale and $k$ is the ratio between the SUSY breaking scale and the scale of the messenger sector. 

For $\sqrt{F} \sim 100\text{--}1000\,\mathrm{TeV}$, the resulting decay length ranges from millimeters to several meters, making the stau observable as a displaced vertex, a kinked track or detector-stable charged particle at FCC-ee~\cite{Mercadante1999,Asai2011}.


\subsection{Signal Samples}
% $e^{+}e^{-} \rightarrow \tilde{\tau}^{-}\tilde{\tau}$
Signal events are generated using \textsc{MadGraph5\_aMC@NLO} v3.2.0~\cite{madgraph} for unpolarized $e^+ e^-$ collisions at $\sqrt{s} = 240$~GeV and $\sqrt{s} = 365$~GeV. The GMSB model was taken by Benjamin Fuks [ADD REFERENCE].
The decay $\tilde{\tau}_1 \rightarrow \tau \tilde{G}$ is enforced with a branching ratio of $100\%$. Each signal sample contains $10^5$ events. Parton-level events are then passed to \textsc{Pythia8}~\cite{pythia8} for parton showering and hadronization. The proper decay length is implemented in PYTHIA by overriding the particle lifetime parameter. Initial- and final-state radiation effects are included to model realistic kinematics in both signal and background events.

The backgrounds considered are chosen based on their large production rates and their potential to mimic the signal topology. The backgrounds considered are shown in


\begin{table}[h]
\centering
\begin{tabular}{lll}
\hline
Process & Decay \\ 
\hline
 $e^+ e^- \to W^+ W^-$ & Inclusive WW \\

$e^+ e^- \to Z Z$ & Inclusive ZZ \\

$e^+ e^- \to ZH$ & $H \to b\bar{b}$ \\

 $e^+ e^- \to \nu_e \bar{\nu}_e H$ 
& $H \to \tau^+ \tau^-$ \\

 $e^+ e^- \to b\bar{b}H$ 
& $H \to \tau^+ \tau^-$ \\
\hline
\end{tabular}
\caption{Background samples considered at $\sqrt{s} = 240$~GeV.}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{lll}
\hline
Dataset & Process & Decay \\
\hline
p8\_ee\_WW\_ecm365 
& $e^+ e^- \to W^+ W^-$ 
& Inclusive WW \\

p8\_ee\_ZZ\_ecm365 
& $e^+ e^- \to Z Z$ 
& Inclusive ZZ \\

p8\_ee\_tt\_ecm365 
& $e^+ e^- \to t\bar{t}$ 
& Inclusive $t\bar{t}$ \\

wzp6\_ee\_nuenueH\_Htautau\_ecm365 
& $e^+ e^- \to \nu_e \bar{\nu}_e H$ 
& $H \to \tau^+ \tau^-$ \\

wzp6\_ee\_bbH\_Htautau\_ecm365 
& $e^+ e^- \to b\bar{b}H$ 
& $H \to \tau^+ \tau^-$ \\

wzp6\_ee\_tautau\_ecm365 
& $e^+ e^- \to \tau^+ \tau^-$ 
& Inclusive $\tau^+\tau^-$ \\
\hline
\end{tabular}
\caption{Background samples considered at $\sqrt{s} = 365$~GeV.}
\end{table}


Each backgrounds sample contained at least $10^5$ unscaled events generated per process. The targeted integrated luminosity for FCC-ee Higgs-strahlung run is 2.7~ab$^{-1}$ at $\sqrt{s} = 240$~GeV and 0.67 ab$^{-1}$ at $\sqrt{s} = 365$~GeV per interaction point~\cite{FeasibilityReport}.  The detector response is modeled using the fast simulation software Delphes with the IDEA FCC-ee card~\cite{delphes}. A \texttt{k4simDelphes} wrapper is used to convert Delphes objects to EDM4HEP format~\cite{Madlener2021}~\cite{Gaede2026_EDM4hep}. The analysis is performed using the \texttt{FCCAnalyses} software framework, which is based on \texttt{RDataFrame}~\cite{FCCAnalyses}. Finally, the \texttt{Combine} tool \cite{combine} is used to compute expected exclusion limits and discovery reach for long-lived staus at FCC-ee.

Previous searches in the maximally mixed scenario exclude staus with proper decay lengths of roughly 20\text{--}330~mm, depending on the stau mass \cite{mykyta}. To explore regions beyond these limits, we simulate staus with masses of 100\text{--}119~GeV and lifetimes ranging from 50~cm up to 50~m, covering both currently unconstrained and experimentally challenging long-lived regimes. The mass is constrained by the available energy of the considered run.

The signal region can be divided according to the tau pair final state. The semileptonic region corresponds to events in which one tau decays hadronically and the other decays to either an electron or a muon, along with the corresponding neutrinos. The hadronic decays of the tau produce final states that include hadrons such as pions and kaons. The charged decay products ($h^{\pm}$) of the tau leptons are referred to as prongs, and hadronic decay modes are characterized by the number of these charged particles, typically resulting in 1-prong (with additional neutral components) and 3-prong topologies. Since the signal process involves $\tilde{\tau} \to \tau \tilde{G}$, a significant fraction of the event energy is carried away by the gravitinos and neutrinos. 



% \input{signal_feynmann}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.90\linewidth]{images/taudecay.png}
%     \caption{Branching ratio of tau leptons \cite{taubranchingratio}.}
%     \label{fig:ditau}
% \end{figure}

